Semi-supervised Classification of Malware Families Under Extreme Class Imbalance via Hierarchical Non-Negative Matrix Factorization with Automatic Model Selection

Identification of the family to which a malware specimen belongs is essential in understanding the behavior of the malware and developing mitigation strategies. Solutions proposed by prior work, however, are often not practicable due to the lack of realistic evaluation factors. These factors include learning under class imbalance, the ability to identify new malware, and the cost of production-quality labeled data. In practice, deployed models face prominent, rare, and new malware families. At the same time, obtaining a large quantity of up-to-date labeled malware for training a model can be expensive. In this paper, we address these problems and propose a novel hierarchical semi-supervised algorithm, which we call the HNMFk Classifier, that can be used in the early stages of the malware family labeling process. Our method is based on non-negative matrix factorization with automatic model selection, that is, with an estimation of the number of clusters. With HNMFk Classifier, we exploit the hierarchical structure of the malware data together with a semi-supervised setup, which enables us to classify malware families under conditions of extreme class imbalance. Our solution can perform abstaining predictions, or rejection option, which yields promising results in the identification of novel malware families and helps with maintaining the performance of the model when a low quantity of labeled data is used. We perform bulk classification of nearly 2,900 both rare and prominent malware families, through static analysis, using nearly 388,000 samples from the EMBER-2018 corpus. In our experiments, we surpass both supervised and semi-supervised baseline models with an F1 score of 0.80.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

all:  ${PDF} ALLSAMPLES


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES:
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut 



clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.75.  \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.76.  Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.77.  Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.78.  Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.
	       

==> notes.tex <==
% \todo[inline]{I'm skipping this section b/c you have a lot of content to migrate down here and will need to edit the whole section to make it cohesive I'm sure. Remember, concise, to the point, and try to make it read as a linear order. THIS is your section to be in teaching mode. -Ed}

%\todo{I'm not sure this paragraph is needed -Ed}Our model performs bulk classification where the known and unknown specimens are provided to the classifier at the same time. This allows us to extract clustering of samples via factorization, where the known specimens are utilized as reference points to classify the unknown samples. Since the factorization is applied both on the unknown and known samples at the same time, we are able to create a semi-supervised setting. In comparison, traditional ML methods use a training set to \todo{tune is very different from train, pick the right word for what you mean. -Ed}tune the model, and perform prediction on the held-out test data. 

\comm{
\comm{
\textit{NMFk} evaluates the stability of the extracted latent components for alternative values for various latent dimension $k$ to estimate the correct latent feature $k$. The workflow for \textit{NMFk} is presented in Figure \ref{fig:NMFk} and the algorithm is presented in Algorithm 1. First, a $r$ random ensemble of matrices $(\ten{X}_1;\ten{X}_2;... ;\ten{X}_r)$ with mean value $\mat{X}$ is generated. Next, each of these ensemble are factorized with NMF consecutively to explore the factors on different latent feature count $k=1,2,3,....N-1$. Thus, for each $k$, corresponding to each ensemble of matrices, we obtain the following:
\begin{equation}
  \begin{array}{l}
    \ten{W} = (\mat{W}_1;\mat{W}_2;... ;\mat{W}_r)\\
    \ten{H} = (\mat{H}_1;\mat{H}_2;... ;\mat{H}_r)
  \end{array}
\end{equation}
where $\ten{W}$ corresponds to the set of features and $\ten{H}$ corresponds to coefficients. Now for each $k$, we first re-order the columns of $W$ for different ensembles so that they are aligned for measure cluster characteristics. The clustering is performed so as to group similar features, which is quantified with cosine similarity. At the end, the clustering results into one column of each solution $\mat{W^k}$ into each of the cluster. Here for each $r$ random ensemble of matrix $X$, we have $r$ different clustered solutions of $\mat{W}$. So, for each $k$ clusters, we have $r$ different data points corresponding to the columns of the features. For each $k$ from clustered ensembles, we compute the mediod of the cluster to extract the representative $\mat{W^*}$. Now, with this $\mat{W^*}$ and original $\mat{X}$, we perfom the regression to return the optimal $\mat{H^*}$. With $\mat{X}$, $\mat{W^*}$ and $\mat{H^*}$, we compute the column-wise reconstruction error between the original $\mat{X}$ and $\mat{W^*} \mat{H^*}$ returning a vector $\vect{C_{err}}=(C_{err_1},C_{err_2},....,C_{err_n})$ where:
\begin{equation}
  \begin{array}{l}
    C_{err_i} = \dfrac{\Vert \mat{X}_{:,i} - \mat{X}^{rec}_{:,i}\Vert}{\Vert\mat{X}_{:,i}\Vert}\\
    \mat{X}^{rec} =\mat{W^*} \mat{H^*}
  \end{array}
\end{equation}

\comm{
There are several unsupervised approaches such as Singular Value Decomposition (SVD), QR decomposition, Cholesky decomposition \cite{CholeskyFactorization}, Principal Component Analysis (PCA), and Independent component analysis (ICA) which are used for applications ranging in solving system of simultaneous linear equations, clustering, and dimensionality reduction. PCA requires orthogonality of the extracted features, while ICA requires their statistical independence \cite{11,12,13}.
\comm{
\todo{This later part is not true, ortogonal independence $\neq$ statistical independence. Do not embellish technical language without good reason. }\todo{response: the sentence wants to tell that PCA->orthogonal independence and ICA->statistically independent as per "respectively" adverb: MB} statistically independent\cite{12,13} respectively, 
}
NMF requires the factors to be non-negative. The non-negativity is crucial for the explainability of the extracted latent patterns. When the factorization produces only non-negative values, the extracted features (the columns of $W$) can only be added (no subtractions are allowed), which requires these features to be sparse and parts of the original data, thus making them easy to understand and interpret \cite{lee1999learning}.}

Next, we employ Silhouette statistics \cite{ROUSSEEUW198753} to determine the cluster stability for each $k$. The Silhouette parameter quantifies the cluster stability in the range $[-1,1]$ where $-1$ corresponds to bad clustering, whereas $1$ correspond to perfect clustering. Finally, we utilize L-statistics to be able to determine the correct $k$ utilizing the silhouette and column-wise reconstruction norm.The L-statistics compares the distributions of column errors corresponding to different $k$ by employing the two-sided Wilcoxon rank-sum test~\cite{Haynes2013}. In an ideal scenario, for optimal k, the reconstruction error is minimal and the silhouette metric is high. 
}

An important problem for matrix and tensor decomposition methods is the determination of the model (or the estimation of the optimal number of latent features). \todo{This task is NP-Hard. Note, that you are also now contradicting all of your OPTIMAL statements, because if you could really find the OPTIMAL number, you would have just revolutionized all of CS and Math by solving an NP-hard problem!!!-Ed}This is a difficult task (in fact it is NP-hard) because the data is constructed with observable features, while the underlying property of the data is hidden. Extracting latent information via estimating the optimal number of clusters  is a significant task. If we estimate the number of clusters to be too high we include noise in our solution (\textit{over-fitting}), and we lose important information if we choose too few clusters to extract  (\textit{under-fitting}). \todo{Which problem, the NP-Hard one? Over/under fitting? }To tackle this problem, Alexandrov et al. introduced a software package named \textit{SmartTensors} which includes factorization methods with automatic model determination \cite{alexandrov2020source, alexandrov2013deciphering, alexandrov2014blind, alexandrov2020patent, nebgen2021neural, SmartTensors}. In its core, \textit{SmartTensors} utilize non-negative matrix factorization with an automatic model determination algorithm (\textit{NMFk}) which applies custom \textit{k-means} clustering and matrix shuffling techniques to obtain \textit{silhouette} and \textit{relative-reconstruction-error} rates, which are used to estimate the optimal number of hidden topics. Our new algorithm, the \textit{hNMFk Classifier}, exploits this automatic model determination obtained by the \textit{NMFk} algorithm to achieve better data separation. \todo{This is a kinda gratuitous over self-citation, I can see a reviewr crabbing. Why don't you pick three relevant/particularly well done ones? -Ed} Since the introduction of \textit{SmartTensors}, the \textit{NMFk} algorithm was used to tackle a number of complex real-world problems, such as decomposition of human  cancer  genomes, defining the cancer mutational signatures, cyber anomaly detection, and text topic modeling  \cite{alexandrov2013signatures, alexandrov2020repertoire, stanev2018unsupervised, lopez2019unsupervised, alexandrov2019nonnegative, karimi2020metabolomics, duc2020trade,
weissman2020increased, zhu2020genomic, vangara2021finding, Vangara2020, Eren2021pyCPAPR, Eren2020lanl}. In addition, the introduction of the distributed version of \textit{NMFk} by Bhattarai et al. has enabled analysis of extremely large datasets \cite{pyDNMFk1, pyDNMFk2, pyDNMFk3}. 

\todo{THIS IS THE WRONG PLACE! 1) Please put figures/algorithms/text just before/right at/just after where they are first reverenced. 2) This is the background section, your approach is not your background! This should be occurring in Section 4!}A diagram illustrating our malware modeling method with \textit{NMFk}, is presented in Figure \ref{fig:NMFk}. \textit{NMFk} includes the following components:
\todo[inline]{This is super hard to follow, in part b/c there is zero given context - we just jumped from background to method. Organize this better, and then again check your statements for 1: Are you actually doing what is claimed (equals mean, or in expectation equals mean?) 2: is it clear/direct (cluster the set of latent malware components is a mouthful at once!) -Ed. 
\\
It looks like the entire rest of this section is a method and should move?}}

\comm{In our methodology, we use NMF, an unsupervised learning technique, to extract the latent features via dimensionality reduction. NMF decomposes given non-negative data matrix $\mat{X}$ into latent factors $\mat{W}$ and $\mat{H}$ which are also non-negative. There are several optimization techniques that can be used to decompose $\mat{X}$ such as multiplicative updates (MU), alternating least squares (ALS), gradient descent, and block coordinate descent. The decomposition is performed with the objective of minimizing the distance between $\mat{X}$ and the reconstruction based on $\mat{W}\mat{H}$ such that:
\begin{equation}
\mat{W}^* \mat{H}^* = \underset{\mat{W},\mat{H}\geq0}{\operatorname{arg\,min}} \,  || \mat{X} - \mat{W}\mat{H} ||_{dist}^2
\end{equation}

Here $dist$  may be Frobenius norm or KL-divergence. In general, NMF minimization with specific distance metrics is equivalent to expectation minimization (EM) algorithm. As a result of this decomposition, columns of $\mat{W}$ correspond to the basis patterns and the rows of $\mat{H}$ correspond to the mixing coefficients such that the linear combination of $\mat{W}$ columns correspond to the column of the $\mat{X}$:
\begin{equation}
\mat{X}_{:,j} = \sum_{s=1}^K \mat{W}_{:,s} \mat{H}_{s,j}
\end{equation}
We utilize the Frobenius norm based multiplicative update for solving NMF problem. The update rules for factor $\mat{W}$ and $\mat{H}$  are given as follows:

\begin{equation}
\begin{split}
\mat{W} = \mat{W}  \frac{\mat{X} \mat{H}^T}{\mat{W} \mat{H} \mat{H}^T+\epsilon}
\\
\mat{H} = \mat{H} \frac{\mat{W}^T \mat{X}}{\mat{W}^T \mat{W} \mat{H}+\epsilon}
\end{split}
\end{equation}
}

\comm{
Similar to the other methods, NMF is also widely used for dimensionality reduction but
\todo{Citation and technical details needed, I have never heard of or seen this argument that NMF can understand structure. -Ed}with an additional capability of dealing with a hierarchical structure. This provides the NMF with the ability to unravel the subgroups within malware clusters by performing hierarchical clustering to identify the underlying hierarchical structure in the data which other methods can not do equally well. It is important to note that other hierarchical clustering frameworks impose a hierarchical structure on data despite the existence of one \cite{guess2002introduction}, but \todo{Citation/explanation needed! I do not believe NMF does that, and I don't think you are talking about NMF. I think you are talking about your approach again, which would make this not background, and also makes this harder to read.  -Ed} \todo{We are speaking about general NMF and with its non-negativity constraint,it provides us this ability. The citation\cite{guess2002introduction} provides details if you go through it.}NMF will avoid such conditions if no hierarchy exists. 
}

% NMF has also been previously applied to the malware classification problem. Ling et al. utilize NMF to detect metamorphic malware (malware with the capability to modify its code during run-time) using static analysis features \cite{ling2019nonnegative}. Ling et al. derive similarity scores of structural patterns from NMF to perform small-scale malware classification, where malware contains data from three families. In their experiments, they choose the number of components for NMF to be $k(n + m) < nm$. Unlike Ling et al., we perform large-scale malware family classification of thousands of families, using hierarchical \textit{NMFk} with the determination of the optimal $k$, or number of components. 

% Hierarchical clustering allows an \todo{What is an error space? -Ed}error space in the optimal cluster selection, as a poorly separated data could be fixed in the successor nodes by the following clusters. This is demonstrated by Gillis et al. when clustering hyperspectral images \cite{gillis2014hierarchical}. In their analysis, rank-two NMF is used at each depth (i.e. split the data into two at each stage, $k=2$). They show that this approach yields good clustering results in a hierarchical setting. We use rank-two clustering in our ablation studies, and show that optimally selecting the number of clusters yield better classification results, although rank-two clustering does yield good classification results that surpass our baseline models.

 % Trigeorgis et al. applied hierarchical Semi-NMF to cluster images of human faces \cite{trigeorgis2014deep}. \textit{Semi-NMF} allows mixed signs in $\mat{X}$ and one of the factors $\mat{W}$ or $\mat{H}$. In their approach, images are grouped using \textit{k-means} clustering from each \textit{Semi-NMF} operation. Using this method, Trigeorgis et al. extracted different categories of facial features at each depth such as pose (angle of the face to the camera), facial expression, and identity features. In their analysis, reconstruction error and clustering accuracy are used to identify the number of components to use during factorization. Alternatively, we optimally choose the number of components using \textit{NMFk}. 

%\todo[inline]{These two papers are good to reference:
%http://cs.ucf.edu/~mohaisen/doc/tr/amal-tr.pdf
%https://link.springer.com/chapter/10.1007/978-3-319-40667-1\_20}

%Malware continues to be a prominent threat to organizations, the public, and national security. Recent reports point out that malware is one of the most frequent and costly cyber threats where a single malware attack, on average, costs \$2.6 million \cite{Ponemon2019}. Approximately, 450,000 new malware samples are reported daily, and the total quantity of malware in the wild has increased by 1178\% in the past 10 years \cite{avtest_2021}. To this end, organizations and AV vendors have started to utilize Machine learning (ML) based automated security systems to combat malware \cite{WinIntel, VirusTotalSangfor, VirusTotalBitdefender, kaspersky_ml}. While ML-based automation can save up to \$3.81 million on data breaches, only about 25\% of organizations have fully-deployed automated incident detection and prevention systems \cite{ibm2021}. With the ever-growing quantity of malware, attacks, and their complexities there is an urgent need to improve existing solutions and their operational architectures to drive the increased adaption of ML-based solutions. 

% Often, ML solutions used to identify malware are supervised models which need an immense quantity of labeled data during training to achieve good performance; however, labeled malware data is expensive to obtain \cite{Raff2020ASO}. At the same time, supervised methods need to be updated regularly as they may generalize poorly to novel malware. To this end, supervised ML models suffer the same issue as the basic signature-based security systems, in which malware authors obfuscate or modify the code and behavior of the malware to bypass these systems \cite{kaspersky_ml, Nguyen2017AttackingML}.

% %\textit{NMFk} estimates the number of malware family clusters which yields better separability of the data. Applying \textit{NMFk} in a hierarchical setting enables analysis of finer-grained details of malware features as we go deeper in the graph, which further enhances the separation of 

% \todo{I share ER's concern over the word optimal.  Are we perhaps offering a heuristic that leads us to optimal or near-optimal clusters, sometimes? we hope?  Also, I need to think about the hierarchical graph.  Are we doing a hierarchical clustering?  I suspect, but do not know, that HC does reach an optimal clustering, with respect to its own objective function, except for accidents due to random tie-breaking.  We should probably discuss this.  CKN}

%\todo[inline]{Its taken 3 pages to get here, it is overall too verbose. For each paragraph/sentence think: 1) what point am I trying to make? 2) How can I make that point quickly and directly. Then write that. }

%\todo[inline]{I think the next 3-4 paragraphs could be just one. We don't need all these details, especially F1 numbers, unless we are going to dig into them. Its hard for the reader to follow all the differences and why the matter. Hit them with short, concise facts. "Several works look at malware family classification, but use only the $\leq 20$ most popular families [cite,cite,cit], where WE DO THE CORRECT/BETTER THING. Hit with the contrast after each point so the reader understands WHY you told them this, and why you are better/smarter! -Ed}

%Zhang et al. perform malware classification, and malware type (such as adware, virus, backdoor, spyware, etc.) classification \cite{8858297}. EMBER-2018 dataset does not contain labels for the malware types; therefore, this study collects type labels using the VirusTotal API. They evaluate malware type classification using supervised models such as \textit{Random Forest} and \textit{LightGBM}, where their highest F1 score of 0.96 is reported with \textit{LightGBM}. However, in their work, the dataset is manually made balanced by removing the rare specimens. This change in the structure of the dataset makes their results unrealistic. 

% Kumar et al. use \textit{XGBoost} to perform malware classification over the entire EMBER-2018 dataset, in a balanced dataset setup \cite{kumar2020malware}. Their work also compares several number of models including \textit{Gaussian Naive Bayes}, \textit{Linear SVC}, \textit{Decision Tree}, and \textit{LightGBM}. Kumar et al. reports their highest F1 score of 0.98 with \textit{XGBoost}.  In comparison to Kumar et al., we perform malware family classification, and perform our experiments in an unbalanced dataset setup.

% There are number of previous work that considered more realistic performance evaluation with their experimental setup. Loi et al. use \textit{LightGBM} to perform malware type and family classification and achieve an accuracy score of 0.89 \cite{loi2021towards}. While our study is performed exclusively over the malicious specimens with the given assumption that the analyst already knows the samples are malware, Loi et al. first classify the samples as malware and benign-ware, and the family classification is only done over the specimens that are predicted to be malware. Their evaluation of the model was limited to the top 20 malware families present in the dataset and the remaining 2,710 families are considered as the \textit{"others"} class. Loi et al. reports that around 63\% of the families are classified with the accuracy score of 0.85, while the remaining (which are heavily represented by the classes collected within \textit{"others"}) are falsely classified due to the supervised method's inability to learn the patterns of these classes from a rare number of specimens. 

%Other datasets have also been used previously in malware family classification. Vinayakumar et al. proposed scalable deep learning-based image processing techniques to perform classification of malware families \cite{8681127}. Their approach considers a two stage approach where the specimens are first classified into benign-ware and malware categories using both static and dynamic analysis techniques prior to malware family classification. This work studies two datasets, Malimg \cite{10.1145/2016904.2016908} and privately collected samples. Malimg contains around 9,000 malware samples from 25 families, and their private dataset consist of 10 malware families each represented by around 1,000 samples. Vinayakumar et al. reaches up to 0.96 F1 score using a \textit{CNN}. Li et al. formulate a malware family classification framework that evaluates several supervised ML models around 2,700 malware samples from VirusShare dataset \cite{8322598, virusShare}. They obtain a F1 score of 0.93 using \textit{Random Forest}; however, this work also sub-samples the dataset and limits the evaluation of the models to only 12 malware families. 

% Hansen et al. also perform malware family classification using \textit{Random Forest}. In this work, the behavioral traces of 270,000 malware samples are collected via Cuckoo Sandbox, and pre-processed via WEKA \cite{frank2005weka}. They report a F1 score of 0.86, but only over the top 5 malware families making around 31,000 samples \cite{7440587}. 

 % Ahmadi et al. also perform malware classification over Malimg dataset using \textit{XGBoost} with bagging to evaluate feature selection and fusion techniques \cite{ahmadi2016novel, Breiman2004BaggingP}. A high accuracy score of 0.99 is reported; however, this work evaluates their approach over only 9 malware families.
 
 % Additionally, supervised methods used in prior work poorly generalize to rare specimens, as pointed out by Loi et al. when they grouped the rare specimens in a single \textit{"others"} class \citep{loi2021towards}. Loi et al. reports that around 63\% of the families are classified with the accuracy score of 0.85, while the remaining (which are heavily represented by the classes collected within \textit{"others"}) are falsely classified due to the supervised method's inability to learn the patterns of these classes from a rare number of specimens.
 
 % Mohaisen et al. use a custom collected dataset consisting of over 115,000 samples, where 2,086 of them are manually labeled as variants of Zeus by domain experts, to perform malware classification and characterization based on dynamic analysis features \citep{MOHAISEN2015251}. Mohaisen et al. introduce a framework where the malware is executed in a virtual environment first, then important malware features are identified, and finally, various supervised models are trained on these features to perform classification. Mohaisen et al. also utilize hierarchical clustering techniques with semi-supervised classification for malware family characterization. Similar to \cite{loi2021towards}, \citep{MOHAISEN2015251} addresses the significant shortcoming of the field by considering unbalanced datasets. To this end, on their large-scale analysis, 7 prominent target families are classified alongside a class \textit{"others"} that represent the remaining of the families consisting of less than 1,000 samples. While Mohaisen et al. does not report their large-scale malware clustering performance and the performance on the \textit{"others"} class, their supervised models achieve F1 scores between 0.85 and 0.91 for the 7 target families. Differently than Mohaisen et al., we do not map the rare specimens into a single \textit{"others"} class, and utilize static analysis based malware features for classification.
 
 % As far as our knowledge, the largest malware family classification work was done by Huang et al. in \cite{huang2016mtnet}. This work uses a proprietary dataset provided by Microsoft Corporation consisting of 6.5 million files to evaluate the performance of their deep neural network-based solution. Huang et all. use dynamic-analysis based features, similar to \citep{MOHAISEN2015251}. In their analysis, 100 malware classes are considered, where 98 are the target malware families selected by security analysts by their prevalence of infection and severity. The other two classes include the one for benign samples, and the \textit{"Generic Malware"} (1.55 million samples) class which is analogous to the \textit{"others"} class from \citep{loi2021towards} and \cite{MOHAISEN2015251}. With this realistic setting, they achieve a low error rate of 2.94\%. Differently than Huang et al., in our analysis, we perform classification for thousands of malware families, although when using a significantly smaller-sized dataset, and when using PE header and malware metadata features.
 
 % Malware characterization is a significant threat in other platforms as well. As Android continues to be one of the most popular mobile operating systems in the market, the threat actors continue to target this platform. Android malware family classification using frequent subgraphs was performed by Fan et al. \citep{8293854}. In their experiments, around 8,000 malware samples, formed from 36 malware families, are classified into their classes with an accuracy score of 0.94.
 
 % In contrast to the prior work, our evaluation of \textit{hNMFk Classifier} is performed using 2,730 malware families (making over 289,000 samples) in the training set to classify 916 families (over 99,000 samples). We do not see over 72\% of the families in the training set again in our test set, and there are 168 malware families (363 samples) that did not exist in our training set. Finally, we include both rare and prominent malware families in our analysis creating an extremely imbalanced dataset. In comparison to prior work, this setup allows our results to be more realistic to what malware analysts would see in the real world.
